Multi-variable Quantification of BDDs in External Memory using Nested Sweeping (Extended Paper)

Previous research on the Adiar BDD package has been successful at designing algorithms capable of handling large Binary Decision Diagrams (BDDs) stored in external memory. To do so, it uses consecutive sweeps through the BDDs to resolve computations. Yet, this approach has kept algorithms for multi-variable quantification, the relational product, and variable reordering out of its scope. In this work, we address this by introducing the nested sweeping framework. Here, multiple concurrent sweeps pass information between eachother to compute the result. We have implemented the framework in Adiar and used it to create a new external memory multi-variable quantification algorithm. Compared to conventional depth-first implementations, Adiar with nested sweeping is able to solve more instances of our benchmarks and/or solve them faster.

==> data/buddy_goe__solved.tex <==
% GoL : None
0.067     0.1940  % 3x3
0.103     0.2039  % 4x3
0.591     0.2403  % 4x4
1.507     0.2230  % 5x4
41.067    0.1986  % 5x5
303.957   0.2311  % 6x5
% GoL : Mirror Vertical
0.054     0.1481  % 3x3
0.077     0.1688  % 4x3
0.173     0.2139  % 4x4
0.261     0.2299  % 5x4
2.519     0.2517  % 5x5
5.684     0.2162  % 6x5
27.544    0.2230  % 6x6
71.650    0.1827  % 7x6
7865.187  0.5110  % 7x7
% GoL : Mirror Quadrant
0.051     0.1569  % 3x3
0.074     0.1622  % 4x3
0.155     0.2000  % 4x4
0.400     0.2400  % 5x4
4.515     0.3045  % 5x5
16.968    0.3679  % 6x5
97.798    0.3384  % 6x6
% GoL : Mirror Diagonal
0.050     0.1200  % 3x3
0.188     0.2074  % 4x4
5.696     0.2795  % 5x5
157.197   0.3508  % 6x6
% GoL : Mirror Double-Diagonal
0.059     0.1695  % 3x3
0.229     0.2489  % 4x4
8.753     0.3593  % 5x5
437.032   0.6831  % 6x6
% GoL : Rotate 90
0.046     0.1522  % 3x3
0.137     0.1971  % 4x4
11.252    0.2745  % 5x5
210.541   0.2848  % 6x6
% GoL : Rotate 180
0.082     0.2195  % 3x3
0.085     0.2000  % 4x3
0.375     0.2373  % 4x4
4.244     0.2988  % 5x4
83.833    0.2846  % 5x5
295.514   0.4001  % 6x5


==> data/buddy_goe__timeouts__truncated.tex <==
% GoL : None
32740.531 5.0000 % 5.2779  % 6x6 % NOTE: Truncated! (mem out...)
% GoL : Mirror Vertical
63937.542 5.0000 % 5.4053  % 8x7 % NOTE: Truncated! (mem out...)
% GoL : Mirror Quadrant
5346.729  5.0000 % 8.0797  % 7x6 % NOTE: Truncated! (mem out...)
% GoL : Mirror Diagonal
10073.097 5.0000 % 17.1546 % 7x7 % NOTE: Truncated! (time out...)
% GoL : Mirror Double-Diagonal

% GoL : Rotate 90

% GoL : Rotate 180
6016.986  5.0000 % 28.7187 % 6x6 % NOTE: Truncated! (mem out...)


==> data/buddy_qbf__solved.tex <==
% QBF : Breakthrough
0.633    0.0506 % 2x4_13
1.937    0.1683 % 2x5_17
2.041    0.1857 % 2x6_15
23.919   0.2819 % 3x4_19
6.910    0.2421 % 3x5_11
2.242    0.2208 % 3x6_9
% QBF : Breakthrough 2nd
0.351    0.0456 % 2x4_8
0.658    0.0699 % 2x5_10
1.629    0.1627 % 2x6_14
4.123    0.2309 % 3x4_12
14.013   0.2499 % 3x5_12
4.488    0.2451 % 3x6_10
% QBF : Connect 4
0.112    0.0089 % 2x2_3_c2
0.174    0.0287 % 3x3_3_c2
0.423    0.0473 % 3x3_9_c3
0.169    0.0355 % 4x4_3_c2
0.509    0.1022 % 4x4_9_c3
2.431    0.2057 % 4x4_15_c4
0.234    0.0598 % 5x5_3_c2
1.441    0.1895 % 5x5_9_c3
4.848    0.2339 % 5x5_11_c4
0.238    0.0630 % 6x6_3_c2
2.697    0.2010 % 6x6_9_c3
13.553   0.2124 % 6x6_11_c4
% QBF : Domineering
0.044    0.0227 % 2x2_2
0.093    0.0215 % 2x3_4
0.096    0.0208 % 2x4_4
0.175    0.0400 % 2x5_6
0.188    0.0479 % 2x6_6
0.053    0.0189 % 3x2_2
0.120    0.0333 % 3x3_4
0.184    0.0217 % 3x4_6
0.307    0.0749 % 3x5_8
0.270    0.1037 % 3x6_6
0.109    0.0183 % 4x2_5
0.195    0.0462 % 4x3_7
0.283    0.0848 % 4x4_8
0.905    0.1834 % 4x5_11
10.130   0.2038 % 4x6_12
0.183    0.0383 % 5x2_6
0.318    0.0755 % 5x3_8
1.067    0.1865 % 5x4_10
20.994   0.2131 % 5x5_13
176.871  0.2779 % 5x6_11
0.185    0.0486 % 6x2_6
0.567    0.1164 % 6x3_10
9.706    0.2060 % 6x4_12
164.585  0.2478 % 6x5_11
% QBF : Evader-Pursuer
0.303    0.0528 % 4x4_3_..
7.019    0.1882 % 4x4_21_..
38.435   0.2028 % 8x8_7_..
% QBF : Evader-Pursuer Dual
0.251    0.0598 % 4x4_2_..
1.998    0.1206 % 4x4_10_..
4.073    0.1844 % 8x8_6_..
922.202  0.9598 % 8x8_10_..
% QBF : Hex
0.274    0.0876 % browne_5x5_07
12.640   0.2081 % browne_5x5_09
213.355  0.5719 % hein_02_5x5-11
843.869  1.6282 % hein_02_5x5-13
0.044    0.0227 % hein_04_3x3-03
0.119    0.0420 % hein_04_3x3-05
3.230    0.1858 % hein_06_4x4-11
4.618    0.2038 % hein_06_4x4-13
0.335    0.0896 % hein_07_4x4-07
1.940    0.1742 % hein_07_4x4-09
6.150    0.1846 % hein_08_5x5-09
25.537   0.1979 % hein_08_5x5-11
0.089    0.0225 % hein_09_4x4-05
0.285    0.0877 % hein_09_4x4-07
99.778   0.2534 % hein_10_5x5-11
473.913  1.0760 % hein_10_5x5-13
9.853    0.2375 % hein_11_5x5-09
97.817   0.2640 % hein_11_5x5-11
0.135    0.0370 % hein_12_4x4-05
0.197    0.0558 % hein_12_4x4-07
0.289    0.0865 % hein_13_5x5-07
11.073   0.2145 % hein_13_5x5-09
0.316    0.0823 % hein_14_5x5-07
20.257   0.2158 % hein_14_5x5-09
71.152   0.1929 % hein_15_5x5-13
108.462  0.1969 % hein_15_5x5-15
123.197  0.2812 % hein_16_5x5-11
498.099  1.0483 % hein_16_5x5-13
2.463    0.1786 % hein_19_5x5-09
12.003   0.1873 % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.123    0.0325 % 3x3_3_domino
0.237    0.0549 % 3x3_5_el
0.547    0.0823 % 3x3_9_elly
0.354    0.0989 % 3x3_9_fatty
0.468    0.0855 % 3x3_9_knobby
0.437    0.0984 % 3x3_9_tic
0.471    0.0849 % 3x3_9_tippy
0.111    0.0450 % 4x4_3_domino
0.263    0.0951 % 4x4_5_el
0.232    0.1034 % 4x4_5_tic
1.422    0.1779 % 4x4_7_elly
12.812   0.2056 % 4x4_9_tippy
70.673   0.2051 % 4x4_11_knobby
149.182  0.2069 % 4x4_13_skinny
168.869  0.3417 % 4x4_15_fatty


==> data/buddy_qbf__timeouts__truncated.tex <==
% QBF : Breakthrough

% QBF : Breakthrough 2nd

% QBF : Connect 4

% QBF : Domineering
2345.901 5.0000 % 18.4151 % 6x6_11   % NOTE: Truncated! (mem out...)
% QBF : Evader-Pursuer
6039.798 5.0000 % 7.1526 % 8x8_11_.. % NOTE: Truncated! (time out...)
% QBF : Evader-Pursuer Dual

% QBF : Hex

% QBF : Tic-Tac-Toe


==> data/cal_goe__solved.tex <==
% GoL : None
0.067     0.1194    % 3x3
0.103     0.1553    % 4x3
0.591     0.8308    % 4x4
1.507     1.7837    % 5x4
41.067    20.2975   % 5x5
% GoL : Mirror Vertical
0.054     0.0926    % 3x3
0.077     0.1039    % 4x3
0.173     0.2139    % 4x4
0.261     0.4674    % 5x4
2.519     2.6757    % 5x5
5.684     56.5116   % 6x5
27.544    100.3563  % 6x6
% GoL : Mirror Quadrant
0.051     0.0980    % 3x3
0.074     0.1081    % 4x3
0.155     0.2000    % 4x4
0.400     0.3250    % 5x4
4.515     0.8563    % 5x5
16.968    1.7135    % 6x5
97.798    2.5041    % 6x6
% GoL : Mirror Diagonal
0.050     0.0800    % 3x3
0.188     0.2447    % 4x4
5.696     0.7886    % 5x5
157.197   190.5265  % 6x6
% GoL : Mirror Double-Diagonal
0.059     0.1017    % 3x3
0.229     0.3188    % 4x4
8.753     1.4213    % 5x5
437.032   11.7976   % 6x6
% GoL : Rotate 90
0.046     0.0870    % 3x3
0.137     0.1971    % 4x4
11.252    1.3454    % 5x5
210.541   3.5599    % 6x6
% GoL : Rotate 180
0.082     0.1707    % 3x3
0.085     0.1294    % 4x3
0.375     0.2987    % 4x4
4.244     0.7158    % 5x4
83.833    1.8363    % 5x5
295.514   4.8434    % 6x5
6016.986  23.7669   % 6x6


==> data/cal_goe__timeouts.tex <==
% GoL : None
303.957   426.3761  % 6x5
32740.531 15.8336   % 6x6
% GoL : Mirror Vertical
71.650    1808.7927 % 7x6
7865.187  32.9554   % 7x7
63937.542 16.2158   % 8x7
% GoL : Mirror Quadrant
5346.729  24.2391   % 7x6
% GoL : Mirror Diagonal
10073.097 51.4638   % 7x7
% GoL : Mirror Double-Diagonal

% GoL : Rotate 90

% GoL : Rotate 180


==> data/cal_qbf__solved.tex <==
% QBF : Breakthrough
0.633    0.0569     % 2x4_13
1.937    1.7135     % 2x5_17
2.041    9.6703     % 2x6_15
23.919   1595.3885  % 3x4_19
6.910    32.3612    % 3x5_11
2.242    9.0874     % 3x6_9
% QBF : Breakthrough 2nd
0.351    0.0342     % 2x4_8
0.658    0.0881     % 2x5_10
1.629    3.6642     % 2x6_14
4.123    10.3357    % 3x4_12
14.013   127.2810   % 3x5_12
4.488    51.4813    % 3x6_10
% QBF : Connect 4
0.112    0.0089     % 2x2_3_c2
0.174    0.0172     % 3x3_3_c2
0.423    0.0378     % 3x3_9_c3
0.169    0.0178     % 4x4_3_c2
0.509    0.1572     % 4x4_9_c3
2.431    4.9079     % 4x4_15_c4
0.234    0.0342     % 5x5_3_c2
1.441    1.8036     % 5x5_9_c3
4.848    10.1698    % 5x5_11_c4
0.238    0.0378     % 6x6_3_c2
2.697    3.3993     % 6x6_9_c3
13.553   8.5785     % 6x6_11_c4
% QBF : Domineering
0.044    0.0227     % 2x2_2
0.093    0.0108     % 2x3_4
0.096    0.0104     % 2x4_4
0.175    0.0171     % 2x5_6
0.188    0.0213     % 2x6_6
0.053    0.0189     % 3x2_2
0.120    0.0167     % 3x3_4
0.184    0.0217     % 3x4_6
0.307    0.0619     % 3x5_8
0.270    0.1259     % 3x6_6
0.109    0.0092     % 4x2_5
0.195    0.0205     % 4x3_7
0.283    0.0777     % 4x4_8
0.905    1.3006     % 4x5_11
10.130   71.8039    % 4x6_12
0.183    0.0164     % 5x2_6
0.318    0.0723     % 5x3_8
1.067    1.6261     % 5x4_10
0.185    0.0216     % 6x2_6
0.567    0.2751     % 6x3_10
9.706    66.0268    % 6x4_12
% QBF : Evader-Pursuer
0.303    0.0396     % 4x4_3_..
% QBF : Evader-Pursuer Dual
0.251    0.0438     % 4x4_2_..
1.998    9.1321     % 4x4_10_..
4.073    3.6428     % 8x8_6_..
% QBF : Hex
0.274    0.0876     % browne_5x5_07
12.640   22.6290    % browne_5x5_09
0.044    0.0227     % hein_04_3x3-03
0.119    0.0168     % hein_04_3x3-05
3.230    19.8248    % hein_06_4x4-11
4.618    40.3837    % hein_06_4x4-13
0.335    0.1284     % hein_07_4x4-07
1.940    6.0387     % hein_07_4x4-09
6.150    13.0859    % hein_08_5x5-09
0.089    0.0112     % hein_09_4x4-05
0.285    0.1123     % hein_09_4x4-07
99.778   318.4258   % hein_10_5x5-11
9.853    35.7668    % hein_11_5x5-09
97.817   346.0878   % hein_11_5x5-11
0.135    0.0148     % hein_12_4x4-05
0.197    0.0254     % hein_12_4x4-07
0.289    0.1073     % hein_13_5x5-07
11.073   23.0985    % hein_13_5x5-09
0.316    0.1044     % hein_14_5x5-07
20.257   35.8433    % hein_14_5x5-09
71.152   1081.1344  % hein_15_5x5-13
123.197  433.1403   % hein_16_5x5-11
2.463    8.0410     % hein_19_5x5-09
12.003   80.2218    % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.123    0.0163     % 3x3_3_domino
0.237    0.0295     % 3x3_5_el
0.547    0.1499     % 3x3_9_elly
0.354    0.1441     % 3x3_9_fatty
0.468    0.1218     % 3x3_9_knobby
0.437    0.1762     % 3x3_9_tic
0.471    0.1210     % 3x3_9_tippy
0.111    0.0180     % 4x4_3_domino
0.263    0.0875     % 4x4_5_el
0.232    0.0991     % 4x4_5_tic
1.422    2.6083     % 4x4_7_elly
12.812   73.8540    % 4x4_9_tippy
70.673   760.7968   % 4x4_11_knobby


==> data/cal_qbf__timeouts__truncated.tex <==
% QBF : Breakthrough

% QBF : Breakthrough 2nd

% QBF : Connect 4

% QBF : Domineering
20.994   85.7388    % 5x5_13
176.871  30.5307    % 5x6_11
164.585  32.8098    % 6x5_11
2345.901 55.2453    % 6x6_11
% QBF : Evader-Pursuer
7.019    4000.00000 % 4x4_21_.. % NOTE: Truncated!
38.435   140.4969   % 8x8_7_..
6039.798 7.1526     % 8x8_11_..
% QBF : Evader-Pursuer Dual
922.202  46.8444    % 8x8_10_..
% QBF : Hex
213.355  607.4383   % hein_02_5x5-11
843.869  307.1567   % hein_02_5x5-13
25.537   70.4860    % hein_08_5x5-11
473.913  546.9358   % hein_10_5x5-13
108.462  1194.8885  % hein_15_5x5-15
498.099  2081.5139  % hein_16_5x5-13
% QBF : Tic-Tac-Toe
149.182  868.7375   % 4x4_13_skinny
168.869  767.4588   % 4x4_15_fatty


==> data/cudd_goe__solved.tex <==
% GoL : None
0.067     0.0597  % 3x3
0.103     0.0874  % 4x3
0.591     0.2386  % 4x4
1.507     0.2475  % 5x4
41.067    0.2554  % 5x5
303.957   0.7125  % 6x5
% GoL : Mirror Vertical
0.054     0.0370  % 3x3
0.077     0.0519  % 4x3
0.173     0.1387  % 4x4
0.261     0.2031  % 5x4
2.519     0.3085  % 5x5
5.684     0.2912  % 6x5
27.544    0.3489  % 6x6
71.650    0.3352  % 7x6
7865.187  1.1631  % 7x7
% GoL : Mirror Quadrant
0.051     0.0392  % 3x3
0.074     0.0541  % 4x3
0.155     0.1226  % 4x4
0.400     0.2250  % 5x4
4.515     0.6255  % 5x5
16.968    0.9855  % 6x5
97.798    0.8843  % 6x6
% GoL : Mirror Diagonal
0.050     0.0200  % 3x3
0.188     0.1543  % 4x4
5.696     0.6891  % 5x5
157.197   1.1144  % 6x6
% GoL : Mirror Double-Diagonal
0.059     0.0508  % 3x3
0.229     0.2096  % 4x4
8.753     0.7883  % 5x5
437.032   1.5955  % 6x6
% GoL : Rotate 90
0.046     0.0217  % 3x3
0.137     0.1168  % 4x4
11.252    0.6800  % 5x5
210.541   0.6988  % 6x6
% GoL : Rotate 180
0.082     0.0976  % 3x3
0.085     0.0824  % 4x3
0.375     0.2133  % 4x4
4.244     0.5429  % 5x4
83.833    0.6742  % 5x5
295.514   0.9392  % 6x5


==> data/cudd_goe__timeouts__truncated.tex <==
% GoL : None
32740.531 5.0000 % 5.2779  % 6x6 % 7x7 % NOTE: (mem out...)
% GoL : Mirror Vertical
63937.542 5.0000 % 5.4053  % 8x7 % 7x7 % NOTE: (time out...)
% GoL : Mirror Quadrant
5346.729  5.0000 % 8.0797  % 7x6 % 7x7 % NOTE: (mem out...)
% GoL : Mirror Diagonal
10073.097 5.0000 % 17.1546 % 7x7 % 7x7 % NOTE: (time out...)
% GoL : Mirror Double-Diagonal

% GoL : Rotate 90

% GoL : Rotate 180
6016.986  5.0000 % 28.7187 % 6x6 % 7x7 % NOTE: (mem out...)


==> data/cudd_qbf__solved.tex <==
% QBF : Breakthrough
0.633    0.0363 % 2x4_13
1.937    0.4027 % 2x5_17
2.041    0.3905 % 2x6_15
23.919   1.3276 % 3x4_19
6.910    0.6343 % 3x5_11
2.242    0.5062 % 3x6_9
% QBF : Breakthrough 2nd
0.351    0.0142 % 2x4_8
0.658    0.0623 % 2x5_10
1.629    0.3180 % 2x6_14
4.123    0.6306 % 3x4_12
14.013   0.7442 % 3x5_12
4.488    0.7155 % 3x6_10
% QBF : Connect 4
0.112    0.0089 % 2x2_3_c2
0.174    0.0057 % 3x3_3_c2
0.423    0.0213 % 3x3_9_c3
0.169    0.0059 % 4x4_3_c2
0.509    0.0923 % 4x4_9_c3
2.431    0.4772 % 4x4_15_c4
0.234    0.0171 % 5x5_3_c2
1.441    0.3921 % 5x5_9_c3
4.848    0.6873 % 5x5_11_c4
0.238    0.0168 % 6x6_3_c2
2.697    0.4839 % 6x6_9_c3
13.553   0.6277 % 6x6_11_c4
% QBF : Domineering
0.044    0.0227 % 2x2_2
0.093    0.0108 % 2x3_4
0.096    0.0104 % 2x4_4
0.175    0.0057 % 2x5_6
0.188    0.0106 % 2x6_6
0.053    0.0189 % 3x2_2
0.120    0.0083 % 3x3_4
0.184    0.0109 % 3x4_6
0.307    0.0391 % 3x5_8
0.270    0.0889 % 3x6_6
0.109    0.0092 % 4x2_5
0.195    0.0103 % 4x3_7
0.283    0.0495 % 4x4_8
0.905    0.3149 % 4x5_11
10.130   0.7496 % 4x6_12
0.183    0.0055 % 5x2_6
0.318    0.0440 % 5x3_8
1.067    0.3730 % 5x4_10
20.994   0.8550 % 5x5_13
176.871  0.9057 % 5x6_11
0.185    0.0108 % 6x2_6
0.567    0.1305 % 6x3_10
9.706    0.7114 % 6x4_12
164.585  0.7912 % 6x5_11
2345.901 1.9376 % 6x6_11
% QBF : Evader-Pursuer
0.303    0.0165 % 4x4_3_..
7.019    0.4620 % 4x4_21_..
38.435   0.6254 % 8x8_7_..
% QBF : Evader-Pursuer Dual
0.251    0.0159 % 4x4_2_..
1.998    0.2172 % 4x4_10_..
4.073    0.3651 % 8x8_6_..
922.202  0.8725 % 8x8_10_..
% QBF : Hex
0.274    0.0438 % browne_5x5_07
12.640   1.0009 % browne_5x5_09
213.355  1.3639 % hein_02_5x5-11
843.869  2.2934 % hein_02_5x5-13
0.044    0.0227 % hein_04_3x3-03
0.119    0.0084 % hein_04_3x3-05
3.230    0.5043 % hein_06_4x4-11
4.618    0.5914 % hein_06_4x4-13
0.335    0.0627 % hein_07_4x4-07
1.940    0.3809 % hein_07_4x4-09
6.150    0.6816 % hein_08_5x5-09
25.537   1.0019 % hein_08_5x5-11
0.089    0.0112 % hein_09_4x4-05
0.285    0.0491 % hein_09_4x4-07
99.778   1.6748 % hein_10_5x5-11
473.913  3.6154 % hein_10_5x5-13
9.853    0.9664 % hein_11_5x5-09
97.817   1.7427 % hein_11_5x5-11
0.135    0.0074 % hein_12_4x4-05
0.197    0.0102 % hein_12_4x4-07
0.289    0.0484 % hein_13_5x5-07
11.073   1.0347 % hein_13_5x5-09
0.316    0.0475 % hein_14_5x5-07
20.257   0.9518 % hein_14_5x5-09
71.152   0.9990 % hein_15_5x5-13
108.462  0.9260 % hein_15_5x5-15
123.197  1.3376 % hein_16_5x5-11
498.099  2.7359 % hein_16_5x5-13
2.463    0.4852 % hein_19_5x5-09
12.003   0.7595 % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.123    0.0081 % 3x3_3_domino
0.237    0.0127 % 3x3_5_el
0.547    0.0768 % 3x3_9_elly
0.354    0.0763 % 3x3_9_fatty
0.468    0.0748 % 3x3_9_knobby
0.437    0.0961 % 3x3_9_tic
0.471    0.0743 % 3x3_9_tippy
0.111    0.0090 % 4x4_3_domino
0.263    0.0456 % 4x4_5_el
0.232    0.0517 % 4x4_5_tic
1.422    0.2954 % 4x4_7_elly
12.812   0.6389 % 4x4_9_tippy
70.673   0.7905 % 4x4_11_knobby
149.182  0.8097 % 4x4_13_skinny
168.869  0.8728 % 4x4_15_fatty


==> data/cudd_qbf__timeouts__truncated.tex <==
% QBF : Breakthrough

% QBF : Breakthrough 2nd

% QBF : Connect 4

% QBF : Domineering

% QBF : Evader-Pursuer
6039.798 5.0000 % 7.1526 % 8x8_11_.. % NOTE: time out...
% QBF : Evader-Pursuer Dual

% QBF : Hex

% QBF : Tic-Tac-Toe


==> data/libbdd_goe__solved.tex <==
% GoL : None
0.067     0.1493  % 3x3
0.103     0.1845  % 4x3
0.591     0.3181  % 4x4
1.507     0.3245  % 5x4
41.067    0.4217  % 5x5
303.957   0.4383  % 6x5
% GoL : Mirror Vertical
0.054     0.1111  % 3x3
0.077     0.1299  % 4x3
0.173     0.2370  % 4x4
0.261     0.2835  % 5x4
2.519     0.3617  % 5x5
5.684     0.3447  % 6x5
27.544    0.4086  % 6x6
71.650    0.3985  % 7x6
7865.187  0.4074  % 7x7
% GoL : Mirror Quadrant
0.051     0.1176  % 3x3
0.074     0.1351  % 4x3
0.155     0.2065  % 4x4
0.400     0.3050  % 5x4
4.515     0.5395  % 5x5
16.968    0.8610  % 6x5
97.798    0.8313  % 6x6
5346.729  0.6352  % 7x6
% GoL : Mirror Diagonal
0.050     0.1000  % 3x3
0.188     0.2234  % 4x4
5.696     0.4256  % 5x5
157.197   0.6047  % 6x6
10073.097 0.5790 % 7x7
% GoL : Mirror Double-Diagonal
0.059     0.1186  % 3x3
0.229     0.2576  % 4x4
8.753     0.5271  % 5x5
437.032   0.7788  % 6x6
% GoL : Rotate 90
0.046     0.1087  % 3x3
0.137     0.1898  % 4x4
11.252    0.4699  % 5x5
210.541   0.5625  % 6x6
% GoL : Rotate 180
0.082     0.1585  % 3x3
0.085     0.1647  % 4x3
0.375     0.2987  % 4x4
4.244     0.5521  % 5x4
83.833    0.7349  % 5x5
295.514   0.8065  % 6x5
6016.986  0.9578  % 6x6


==> data/libbdd_goe__timeouts__truncated.tex <==
% GoL : None
32740.531 5.0000 % 5.2779  % 6x6 % NOTE: mem out...
% GoL : Mirror Vertical
63937.542 5.0000 % 5.4053  % 8x7 % NOTE: mem out...
% GoL : Mirror Quadrant

% GoL : Mirror Diagonal

% GoL : Mirror Double-Diagonal

% GoL : Rotate 90

% GoL : Rotate 180


==> data/libbdd_qbf__solved.tex <==
% QBF : Breakthrough
0.633    0.0664 % 2x4_13
1.937    0.2731 % 2x5_17
2.041    0.2994 % 2x6_15
23.919   0.6760 % 3x4_19
6.910    0.4839 % 3x5_11
2.242    0.3479 % 3x6_9
% QBF : Breakthrough 2nd
0.351    0.0427 % 2x4_8
0.658    0.1003 % 2x5_10
1.629    0.2455 % 2x6_14
4.123    0.4317 % 3x4_12
14.013   0.5561 % 3x5_12
4.488    0.4697 % 3x6_10
% QBF : Connect 4
0.112    0.0089 % 2x2_3_c2
0.174    0.0172 % 3x3_3_c2
0.423    0.0496 % 3x3_9_c3
0.169    0.0178 % 4x4_3_c2
0.509    0.1297 % 4x4_9_c3
2.431    0.3521 % 4x4_15_c4
0.234    0.0470 % 5x5_3_c2
1.441    0.3234 % 5x5_9_c3
4.848    0.4986 % 5x5_11_c4
0.238    0.0504 % 6x6_3_c2
2.697    0.3597 % 6x6_9_c3
13.553   0.4854 % 6x6_11_c4
% QBF : Domineering
0.044    0.0227 % 2x2_2
0.093    0.0108 % 2x3_4
0.096    0.0104 % 2x4_4
0.175    0.0286 % 2x5_6
0.188    0.0319 % 2x6_6
0.053    0.0189 % 3x2_2
0.120    0.0167 % 3x3_4
0.184    0.0326 % 3x4_6
0.307    0.0912 % 3x5_8
0.270    0.1185 % 3x6_6
0.109    0.0092 % 4x2_5
0.195    0.0308 % 4x3_7
0.283    0.0848 % 4x4_8
0.905    0.3083 % 4x5_11
10.130   0.5142 % 4x6_12
0.183    0.0219 % 5x2_6
0.318    0.0849 % 5x3_8
1.067    0.2962 % 5x4_10
20.994   0.5952 % 5x5_13
176.871  0.6900 % 5x6_11
0.185    0.0270 % 6x2_6
0.567    0.1799 % 6x3_10
9.706    0.5195 % 6x4_12
164.585  0.6602 % 6x5_11
2345.901 0.6701 % 6x6_11
% QBF : Evader-Pursuer
0.303    0.0396 % 4x4_3_..
7.019    0.3808 % 4x4_21_..
38.435   0.5065 % 8x8_7_..
% QBF : Evader-Pursuer Dual
0.251    0.0438 % 4x4_2_..
1.998    0.1922 % 4x4_10_..
4.073    0.3452 % 8x8_6_..
922.202  0.5707 % 8x8_10_..
% QBF : Hex
0.274    0.0912 % browne_5x5_07
12.640   0.4095 % browne_5x5_09
213.355  0.5333 % hein_02_5x5-11
843.869  0.6667 % hein_02_5x5-13
0.044    0.0227 % hein_04_3x3-03
0.119    0.0168 % hein_04_3x3-05
3.230    0.3440 % hein_06_4x4-11
4.618    0.4331 % hein_06_4x4-13
0.335    0.1015 % hein_07_4x4-07
1.940    0.3015 % hein_07_4x4-09
6.150    0.3216 % hein_08_5x5-09
25.537   0.4587 % hein_08_5x5-11
0.089    0.0112 % hein_09_4x4-05
0.285    0.0947 % hein_09_4x4-07
99.778   0.5288 % hein_10_5x5-11
473.913  0.6078 % hein_10_5x5-13
9.853    0.4691 % hein_11_5x5-09
97.817   0.5281 % hein_11_5x5-11
0.135    0.0222 % hein_12_4x4-05
0.197    0.0406 % hein_12_4x4-07
0.289    0.0969 % hein_13_5x5-07
11.073   0.4055 % hein_13_5x5-09
0.316    0.0918 % hein_14_5x5-07
20.257   0.4557 % hein_14_5x5-09
71.152   0.5402 % hein_15_5x5-13
108.462  0.5831 % hein_15_5x5-15
123.197  0.5489 % hein_16_5x5-11
498.099  0.6319 % hein_16_5x5-13
2.463    0.2952 % hein_19_5x5-09
12.003   0.4081 % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.123    0.0163 % 3x3_3_domino
0.237    0.0380 % 3x3_5_el
0.547    0.1152 % 3x3_9_elly
0.354    0.1328 % 3x3_9_fatty
0.468    0.1175 % 3x3_9_knobby
0.437    0.1304 % 3x3_9_tic
0.471    0.1168 % 3x3_9_tippy
0.111    0.0270 % 4x4_3_domino
0.263    0.0875 % 4x4_5_el
0.232    0.0905 % 4x4_5_tic
1.422    0.2616 % 4x4_7_elly
12.812   0.4094 % 4x4_9_tippy
70.673   0.5651 % 4x4_11_knobby
149.182  0.5679 % 4x4_13_skinny
168.869  0.6369 % 4x4_15_fatty


==> data/libbdd_qbf__timeouts__truncated.tex <==
% QBF : Breakthrough

% QBF : Breakthrough 2nd

% QBF : Connect 4

% QBF : Domineering

% QBF : Evader-Pursuer
6039.798 5.0000 % 7.1526 % 8x8_11_.. % NOTE: (mem out...)
% QBF : Evader-Pursuer Dual

% QBF : Hex

% QBF : Tic-Tac-Toe


==> data/oxidd_goe__solved.tex <==
% GoL : None
0.067     0.1194  % 3x3
0.103     0.1748  % 4x3
0.591     0.3418  % 4x4
1.507     0.3119  % 5x4
41.067    0.2968  % 5x5
303.957   0.2652  % 6x5
% GoL : Mirror Vertical
0.054     0.0741  % 3x3
0.077     0.1039  % 4x3
0.173     0.2486  % 4x4
0.261     0.2912  % 5x4
2.519     0.3545  % 5x5
5.684     0.3001  % 6x5
27.544    0.3344  % 6x6
71.650    0.2731  % 7x6
7865.187  2.5882  % 7x7
% GoL : Mirror Quadrant
0.051     0.0980  % 3x3
0.074     0.1081  % 4x3
0.155     0.2129  % 4x4
0.400     0.3275  % 5x4
4.515     0.4939  % 5x5
16.968    0.6576  % 6x5
97.798    0.6001  % 6x6
% GoL : Mirror Diagonal
0.050     0.0600  % 3x3
0.188     0.2394  % 4x4
5.696     0.4724  % 5x5
157.197   0.4835  % 6x6
% GoL : Mirror Double-Diagonal
0.059     0.0847  % 3x3
0.229     0.3188  % 4x4
8.753     0.5596  % 5x5
437.032   0.6271  % 6x6
% GoL : Rotate 90
0.046     0.0652  % 3x3
0.137     0.1825  % 4x4
11.252    0.4525  % 5x5
210.541   0.4310  % 6x6
% GoL : Rotate 180
0.082     0.1707  % 3x3
0.085     0.1529  % 4x3
0.375     0.3280  % 4x4
4.244     0.4764  % 5x4
83.833    0.4852  % 5x5
295.514   0.5875  % 6x5
6016.986  0.9264  % 6x6


==> data/oxidd_goe__timeouts__truncated.tex <==
% GoL : None
32740.531 5.0000 % 5.2779  % 6x6 % NOTE: mem out...
% GoL : Mirror Vertical
63937.542 5.0000 % 5.4053  % 8x7 % NOTE: time out...
% GoL : Mirror Quadrant
5346.729  5.0000 % 8.0797  % 7x6 % NOTE: mem out...
% GoL : Mirror Diagonal
10073.097 5.0000 % 17.1546 % 7x7 % NOTE: time out...
% GoL : Mirror Double-Diagonal

% GoL : Rotate 90

% GoL : Rotate 180


==> data/oxidd_qbf__solved.tex <==
% QBF : Breakthrough
0.633    0.0553 % 2x4_13
1.937    0.2963 % 2x5_17
2.041    0.3146 % 2x6_15
23.919   0.6350 % 3x4_19
6.910    0.4540 % 3x5_11
2.242    0.3515 % 3x6_9
% QBF : Breakthrough 2nd
0.351    0.0285 % 2x4_8
0.658    0.0836 % 2x5_10
1.629    0.2505 % 2x6_14
4.123    0.4196 % 3x4_12
14.013   0.4901 % 3x5_12
4.488    0.4184 % 3x6_10
% QBF : Connect 4
0.112    0.0089 % 2x2_3_c2
0.174    0.0115 % 3x3_3_c2
0.423    0.0355 % 3x3_9_c3
0.169    0.0118 % 4x4_3_c2
0.509    0.1356 % 4x4_9_c3
2.431    0.3723 % 4x4_15_c4
0.234    0.0342 % 5x5_3_c2
1.441    0.3005 % 5x5_9_c3
4.848    0.4313 % 5x5_11_c4
0.238    0.0378 % 6x6_3_c2
2.697    0.3496 % 6x6_9_c3
13.553   0.4062 % 6x6_11_c4
% QBF : Domineering
0.044    0.0227 % 2x2_2
0.093    0.0108 % 2x3_4
0.096    0.0104 % 2x4_4
0.175    0.0171 % 2x5_6
0.188    0.0213 % 2x6_6
0.053    0.0189 % 3x2_2
0.120    0.0083 % 3x3_4
0.184    0.0217 % 3x4_6
0.307    0.0684 % 3x5_8
0.270    0.1074 % 3x6_6
0.109    0.0092 % 4x2_5
0.195    0.0205 % 4x3_7
0.283    0.0777 % 4x4_8
0.905    0.2928 % 4x5_11
10.130   0.4240 % 4x6_12
0.183    0.0164 % 5x2_6
0.318    0.0660 % 5x3_8
1.067    0.2746 % 5x4_10
20.994   0.4678 % 5x5_13
176.871  0.4354 % 5x6_11
0.185    0.0216 % 6x2_6
0.567    0.1658 % 6x3_10
9.706    0.4158 % 6x4_12
164.585  0.4471 % 6x5_11
2345.901 1.2718 % 6x6_11
% QBF : Evader-Pursuer
0.303    0.0297 % 4x4_3_..
7.019    0.3026 % 4x4_21_..
38.435   0.3820 % 8x8_7_..
% QBF : Evader-Pursuer Dual
0.251    0.0319 % 4x4_2_..
1.998    0.1692 % 4x4_10_..
4.073    0.3030 % 8x8_6_..
922.202  0.4179 % 8x8_10_..
% QBF : Hex
0.274    0.0766 % browne_5x5_07
12.640   0.3735 % browne_5x5_09
213.355  0.3960 % hein_02_5x5-11
843.869  0.8746 % hein_02_5x5-13
0.044    0.0227 % hein_04_3x3-03
0.119    0.0084 % hein_04_3x3-05
3.230    0.3362 % hein_06_4x4-11
4.618    0.3909 % hein_06_4x4-13
0.335    0.0896 % hein_07_4x4-07
1.940    0.2964 % hein_07_4x4-09
6.150    0.3109 % hein_08_5x5-09
25.537   0.3708 % hein_08_5x5-11
0.089    0.0112 % hein_09_4x4-05
0.285    0.0807 % hein_09_4x4-07
99.778   0.4033 % hein_10_5x5-11
473.913  0.4535 % hein_10_5x5-13
9.853    0.4208 % hein_11_5x5-09
97.817   0.3964 % hein_11_5x5-11
0.135    0.0148 % hein_12_4x4-05
0.197    0.0254 % hein_12_4x4-07
0.289    0.0830 % hein_13_5x5-07
11.073   0.3533 % hein_13_5x5-09
0.316    0.0791 % hein_14_5x5-07
20.257   0.3759 % hein_14_5x5-09
71.152   0.4082 % hein_15_5x5-13
108.462  0.4298 % hein_15_5x5-15
123.197  0.4103 % hein_16_5x5-11
498.099  0.5049 % hein_16_5x5-13
2.463    0.3037 % hein_19_5x5-09
12.003   0.3621 % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.123    0.0163 % 3x3_3_domino
0.237    0.0295 % 3x3_5_el
0.547    0.1079 % 3x3_9_elly
0.354    0.1158 % 3x3_9_fatty
0.468    0.1090 % 3x3_9_knobby
0.437    0.1236 % 3x3_9_tic
0.471    0.1062 % 3x3_9_tippy
0.111    0.0180 % 4x4_3_domino
0.263    0.0951 % 4x4_5_el
0.232    0.0991 % 4x4_5_tic
1.422    0.3017 % 4x4_7_elly
12.812   0.4058 % 4x4_9_tippy
70.673   0.4320 % 4x4_11_knobby
149.182  0.4505 % 4x4_13_skinny
168.869  0.5240 % 4x4_15_fatty


==> data/oxidd_qbf__timeouts__truncated.tex <==
% QBF : Breakthrough

% QBF : Breakthrough 2nd

% QBF : Connect 4

% QBF : Domineering

% QBF : Evader-Pursuer
6039.798 5.0000 % 7.1526 % 8x8_11_.. % NOTE: time out...
% QBF : Evader-Pursuer Dual

% QBF : Hex

% QBF : Tic-Tac-Toe



==> data/singleton_goe.tex <==
% GoL : None
0.089     0.7528 % 3x3
0.140     0.7357 % 4x3
0.972     0.6080 % 4x4
2.670     0.5644 % 5x4
50.072    0.8202 % 5x5
310.237   0.9798 % 6x5
30926.267 1.0587 % 6x6
% GoL : Mirror Vertical
0.070     0.7714 % 3x3
0.100     0.7700 % 4x3
0.264     0.6553 % 4x4
0.515     0.5068 % 5x4
5.249     0.4799 % 5x5
11.113    0.5115 % 6x5
58.112    0.4740 % 6x6
122.830   0.5833 % 7x6
8666.484  0.9075 % 7x7
61765.369 1.0352 % 8x7
% GoL : Mirror Quadrant
0.069     0.7391 % 3x3
0.095     0.7789 % 4x3
0.211     0.7346 % 4x4
0.734     0.5450 % 5x4
10.239    0.4410 % 5x5
59.596    0.2847 % 6x5
340.575   0.2872 % 6x6
12886.406 0.4149 % 7x6
% GoL : Mirror Diagonal
0.068     0.7353 % 3x3
0.302     0.6225 % 4x4
11.609    0.4907 % 5x5
458.528   0.3428 % 6x6
20922.406 0.4815 % 7x7
% GoL : Mirror Double Diagonal
0.066     0.8939 % 3x3
0.323     0.7090 % 4x4
16.847    0.5196 % 5x5
1082.230  0.4038 % 6x6
% GoL : Rotate 90
0.065     0.7077 % 3x3
0.190     0.7211 % 4x4
16.726    0.6727 % 5x5
455.303   0.4624 % 6x6
% GoL : Rotate 180
0.107     0.7664 % 3x3
0.120     0.7083 % 4x3
0.614     0.6107 % 4x4
9.721     0.4366 % 5x4
199.035   0.4212 % 5x5
848.703   0.3482 % 6x5
17721.873 0.3395 % 6x6


==> data/singleton_qbf.tex <==
% QBF : Breakthrough
0.905    0.6994 % 2x4_13
6.589    0.2940 % 2x5_17
6.439    0.3170 % 2x6_15
140.052  0.1708 % 3x4_19
24.225   0.2852 % 3x5_11
4.029    0.5565 % 3x6_9
% QBF : Breakthrough 2nd
0.419    0.8377 % 2x4_8
0.938    0.7015 % 2x5_10
4.321    0.3770 % 2x6_14
15.326   0.2690 % 3x4_12
56.614   0.2475 % 3x5_12
9.716    0.4619 % 3x6_10
% QBF : Connect 4
0.121    0.9256 % 2x2_3_c2
0.192    0.9063 % 3x3_3_c2
0.528    0.8011 % 3x3_9_c3
0.185    0.9135 % 4x4_3_c2
0.867    0.5871 % 4x4_9_c3
5.560    0.4372 % 4x4_15_c4
0.255    0.9176 % 5x5_3_c2
3.373    0.4272 % 5x5_9_c3
8.696    0.5575 % 5x5_11_c4
0.263    0.9049 % 6x6_3_c2
7.370    0.3659 % 6x6_9_c3
24.804   0.5464 % 6x6_11_c4
% QBF : Domineering
0.045    0.9778 % 2x2_2
0.099    0.9394 % 2x3_4
0.109    0.8807 % 2x4_4
0.195    0.8974 % 2x5_6
0.213    0.8826 % 2x6_6
0.054    0.9815 % 3x2_2
0.134    0.8955 % 3x3_4
0.207    0.8889 % 3x4_6
0.401    0.7656 % 3x5_8
0.358    0.7542 % 3x6_6
0.116    0.9397 % 4x2_5
0.223    0.8744 % 4x3_7
0.400    0.7075 % 4x4_8
2.360    0.3835 % 4x5_11
35.054   0.2890 % 4x6_12
0.200    0.9150 % 5x2_6
0.403    0.7891 % 5x3_8
2.353    0.4535 % 5x4_10
72.629   0.2891 % 5x5_13
420.477  0.4206 % 5x6_11
0.206    0.8981 % 6x2_6
0.833    0.6807 % 6x3_10
32.631   0.2974 % 6x4_12
412.219  0.3993 % 6x5_11
4904.240 0.4783 % 6x6_11
% QBF : Evader-Pursuer
0.320    0.9469 % 4x4_3_..
8.931    0.7859 % 4x4_21_..
36.786   1.0448 % 8x8_7_..
5618.784 1.0749 % 8x8_11_..
% QBF : Evader-Pursuer Dual
0.265    0.9472 % 4x4_2_..
2.573    0.7765 % 4x4_10_..
4.355    0.9352 % 8x8_6_..
881.284  1.0464 % 8x8_10_..
% QBF : Hex
0.358    0.7654 % browne_5x5_07
23.739   0.5325 % browne_5x5_09
491.419  0.4342 % hein_02_5x5-11
2609.547 0.3234 % hein_02_5x5-13
0.047    0.9362 % hein_04_3x3-03
0.137    0.8686 % hein_04_3x3-05
8.811    0.3666 % hein_06_4x4-11
15.332   0.3012 % hein_06_4x4-13
0.464    0.7220 % hein_07_4x4-07
4.807    0.4036 % hein_07_4x4-09
10.734   0.5729 % hein_08_5x5-09
63.525   0.4020 % hein_08_5x5-11
0.100    0.8900 % hein_09_4x4-05
0.394    0.7234 % hein_09_4x4-07
221.110  0.4513 % hein_10_5x5-11
1094.754 0.4329 % hein_10_5x5-13
22.471   0.4385 % hein_11_5x5-09
202.324  0.4835 % hein_11_5x5-11
0.157    0.8599 % hein_12_4x4-05
0.237    0.8312 % hein_12_4x4-07
0.394    0.7335 % hein_13_5x5-07
20.916   0.5294 % hein_13_5x5-09
0.424    0.7453 % hein_14_5x5-07
39.790   0.5091 % hein_14_5x5-09
203.405  0.3498 % hein_15_5x5-13
350.622  0.3093 % hein_15_5x5-15
295.844  0.4164 % hein_16_5x5-11
1321.432 0.3769 % hein_16_5x5-13
5.528    0.4455 % hein_19_5x5-09
32.295   0.3717 % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.133   0.9248 % 3x3_3_domino
0.275   0.8618 % 3x3_5_el
0.882   0.6202 % 3x3_9_elly
0.518   0.6834 % 3x3_9_fatty
0.729   0.6420 % 3x3_9_knobby
0.730   0.5986 % 3x3_9_tic
0.729   0.6461 % 3x3_9_tippy
0.125   0.8880 % 4x4_3_domino
0.329   0.7994 % 4x4_5_el
0.291   0.7973 % 4x4_5_tic
2.486   0.5720 % 4x4_7_elly
31.951  0.4010 % 4x4_9_tippy
218.844 0.3229 % 4x4_11_knobby
403.217 0.3700 % 4x4_13_skinny
406.470 0.4155 % 4x4_15_fatty


==> data/sylvan_goe__solved.tex <==
% GoL : None
0.067     0.3433  % 3x3
0.103     0.2913  % 4x3
0.591     0.2437  % 4x4
1.507     0.1666  % 5x4
41.067    0.1899  % 5x5
303.957   0.0925  % 6x5
32740.531 0.1606  % 6x6
% GoL : Mirror Vertical
0.054     0.3519  % 3x3
0.077     0.2857  % 4x3
0.173     0.2601  % 4x4
0.261     0.2567  % 5x4
2.519     0.2231  % 5x5
5.684     0.2437  % 6x5
27.544    0.3498  % 6x6
71.650    0.2049  % 7x6
7865.187  0.1590  % 7x7
63937.542 0.2431  % 8x7
% GoL : Mirror Quadrant
0.051     0.3725  % 3x3
0.074     0.2973  % 4x3
0.155     0.2581  % 4x4
0.400     0.2450  % 5x4
4.515     0.5477  % 5x5
16.968    0.8530  % 6x5
97.798    0.8160  % 6x6
5346.729  1.5300  % 7x6
% GoL : Mirror Diagonal
0.050     0.3600  % 3x3
0.188     0.2766  % 4x4
5.696     1.0314  % 5x5
157.197   4.0595  % 6x6
% GoL : Mirror Double-Diagonal
0.059     0.3390  % 3x3
0.229     0.3013  % 4x4
8.753     0.7231  % 5x5
437.032   0.9938  % 6x6
% GoL : Rotate 90
0.046     0.3913  % 3x3
0.137     0.2774  % 4x4
11.252    0.6991  % 5x5
210.541   0.7102  % 6x6
% GoL : Rotate 180
0.082     0.3415  % 3x3
0.085     0.3176  % 4x3
0.375     0.3147  % 4x4
4.244     0.3782  % 5x4
83.833    0.5580  % 5x5
295.514   0.7580  % 6x5
6016.986  0.9037  % 6x6


==> data/sylvan_goe__timeouts__truncated.tex <==
% GoL : None

% GoL : Mirror Vertical

% GoL : Mirror Quadrant

% GoL : Mirror Diagonal
10073.097 5.0000 % 17.1546 % 7x7 % NOTE: Time out...
% GoL : Mirror Double-Diagonal

% GoL : Rotate 90

% GoL : Rotate 180


==> data/sylvan_qbf.tex <==
% QBF : Breakthrough
0.633    0.0664 % 2x4_13
1.937    0.3067 % 2x5_17
2.041    0.3082 % 2x6_15
23.919   1.1470 % 3x4_19
6.910    0.7370 % 3x5_11
2.242    0.5397 % 3x6_9
% QBF : Breakthrough 2nd
0.351    0.0684 % 2x4_8
0.658    0.0836 % 2x5_10
1.629    0.2204 % 2x6_14
4.123    0.6726 % 3x4_12
14.013   0.8658 % 3x5_12
4.488    0.8048 % 3x6_10
% QBF : Connect 4
0.112    0.0982 % 2x2_3_c2
0.174    0.0920 % 3x3_3_c2
0.423    0.0638 % 3x3_9_c3
0.169    0.0947 % 4x4_3_c2
0.509    0.1277 % 4x4_9_c3
2.431    0.3501 % 4x4_15_c4
0.234    0.0897 % 5x5_3_c2
1.441    0.2505 % 5x5_9_c3
4.848    0.6803 % 5x5_11_c4
0.238    0.0924 % 6x6_3_c2
2.697    0.3478 % 6x6_9_c3
13.553   0.7021 % 6x6_11_c4
% QBF : Domineering
0.044    0.1818 % 2x2_2
0.093    0.1398 % 2x3_4
0.096    0.1354 % 2x4_4
0.175    0.0971 % 2x5_6
0.188    0.1011 % 2x6_6
0.053    0.1698 % 3x2_2
0.120    0.1333 % 3x3_4
0.184    0.0978 % 3x4_6
0.307    0.1010 % 3x5_8
0.270    0.1370 % 3x6_6
0.109    0.1284 % 4x2_5
0.195    0.0923 % 4x3_7
0.283    0.1131 % 4x4_8
0.905    0.2320 % 4x5_11
10.130   0.6263 % 4x6_12
0.183    0.0929 % 5x2_6
0.318    0.0975 % 5x3_8
1.067    0.2390 % 5x4_10
20.994   0.8094 % 5x5_13
176.871  1.0859 % 5x6_11
0.185    0.0973 % 6x2_6
0.567    0.1429 % 6x3_10
9.706    0.6727 % 6x4_12
164.585  1.0379 % 6x5_11
2345.901 1.6011 % 6x6_11
% QBF : Evader-Pursuer
0.303    0.0759 % 4x4_3_..
7.019    0.4790 % 4x4_21_..
38.435   0.7460 % 8x8_7_..
6039.798 1.3947 % 8x8_11_..
% QBF : Evader-Pursuer Dual
0.251    0.0876 % 4x4_2_..
1.998    0.1537 % 4x4_10_..
4.073    0.4240 % 8x8_6_..
922.202  1.0922 % 8x8_10_..
% QBF : Hex
0.274    0.1095 % browne_5x5_07
12.640   0.7740 % browne_5x5_09
213.355  1.4908 % hein_02_5x5-11
843.869  1.5368 % hein_02_5x5-13
0.044    0.1818 % hein_04_3x3-03
0.119    0.1261 % hein_04_3x3-05
3.230    0.4136 % hein_06_4x4-11
4.618    0.5715 % hein_06_4x4-13
0.335    0.1104 % hein_07_4x4-07
1.940    0.2526 % hein_07_4x4-09
6.150    0.6902 % hein_08_5x5-09
25.537   1.2266 % hein_08_5x5-11
0.089    0.1461 % hein_09_4x4-05
0.285    0.1123 % hein_09_4x4-07
99.778   1.5703 % hein_10_5x5-11
473.913  1.6113 % hein_10_5x5-13
9.853    0.9124 % hein_11_5x5-09
97.817   1.5513 % hein_11_5x5-11
0.135    0.1185 % hein_12_4x4-05
0.197    0.0914 % hein_12_4x4-07
0.289    0.1142 % hein_13_5x5-07
11.073   0.8593 % hein_13_5x5-09
0.316    0.1076 % hein_14_5x5-07
20.257   1.0175 % hein_14_5x5-09
71.152   1.1081 % hein_15_5x5-13
108.462  0.9307 % hein_15_5x5-15
123.197  1.4656 % hein_16_5x5-11
498.099  1.5705 % hein_16_5x5-13
2.463    0.2753 % hein_19_5x5-09
12.003   0.7926 % hein_19_5x5-11
% QBF : Tic-Tac-Toe
0.123    0.1301 % 3x3_3_domino
0.237    0.0886 % 3x3_5_el
0.547    0.1060 % 3x3_9_elly
0.354    0.1299 % 3x3_9_fatty
0.468    0.1132 % 3x3_9_knobby
0.437    0.1327 % 3x3_9_tic
0.471    0.1125 % 3x3_9_tippy
0.111    0.1441 % 4x4_3_domino
0.263    0.1255 % 4x4_5_el
0.232    0.1379 % 4x4_5_tic
1.422    0.2475 % 4x4_7_elly
12.812   0.8183 % 4x4_9_tippy
70.673   0.9742 % 4x4_11_knobby
149.182  1.0501 % 4x4_13_skinny
168.869  1.0163 % 4x4_15_fatty


==> tikz/nested_cases__tree.tex <==
% triangle
\draw (0,0) -- (3,4) -- (6,0) -- cycle;


==> tikz/nested_cases__xi.tex <==
% level x_i
\draw[densely dotted] (2,2.65) -- (4,2.65);
\node at (1.75,2.82) {$x_i$};
\draw[densely dotted] (2.25,3) -- (3.75,3);


==> tikz/nested_cases__xj.tex <==
% level x_j
\draw[red, densely dotted] (1.13,1.5) -- (4.87,1.5);
\node[red] at (0.9,1.67) {$x_j$};
\draw[red, densely dotted] (1.39,1.85) -- (4.6,1.86);
